Towards Scalable 3D Anomaly Detection and Localization: A Benchmark via 3D Anomaly Synthesis and A Self-Supervised Learning Network

Recently, 3D anomaly detection, a crucial problem involving fine-grained geometry discrimination, is getting more attention. However, the lack of abundant real 3D anomaly data limits the scalability of current models. To enable scalable anomaly data collection, we propose a 3D anomaly synthesis pipeline to adapt existing large-scale 3Dmodels for 3D anomaly detection. Specifically, we construct a synthetic dataset, i.e., Anomaly-ShapeNet, basedon ShapeNet. Anomaly-ShapeNet consists of 1600 point cloud samples under 40 categories, which provides a rich and varied collection of data, enabling efficient training and enhancing adaptability to industrial scenarios. Meanwhile,to enable scalable representation learning for 3D anomaly localization, we propose a self-supervised method, i.e., Iterative Mask Reconstruction Network (IMRNet). During training, we propose a geometry-aware sample module to preserve potentially anomalous local regions during point cloud down-sampling. Then, we randomly mask out point patches and sent the visible patches to a transformer for reconstruction-based self-supervision. During testing, the point cloud repeatedly goes through the Mask Reconstruction Network, with each iteration's output becoming the next input. By merging and contrasting the final reconstructed point cloud with the initial input, our method successfully locates anomalies. Experiments show that IMRNet outperforms previous state-of-the-art methods, achieving 66.1% in I-AUC on Anomaly-ShapeNet dataset and 72.5% in I-AUC on Real3D-AD dataset. Our dataset will be released at https://github.com/Chopper-233/Anomaly-ShapeNet

==> latex/figures/Anomalymap/shapenet.tex <==
\begin{figure}[t]
\begin{center}
\subfloat{\includegraphics[width=0.95\linewidth]{latex/figures/Anomalymap/anomaly-result.png}}\end{center}
\vspace{-7mm}
\caption{\textbf{Qualitative results visualization of anomaly detection and localization performance on Anomaly ShapeNet.}
% 
% 
% We note that the synthesized blurry hand image contains multiple annotations from 3D GTs of \emph{1st}, \emph{3rd}, and \emph{5th} sharp frames.

\vspace{-4mm}
\label{fig:Visual-AS}
\end{figure}

==> latex/sections/figures/vis.tex <==
\begin{figure}
\begin{center}
\hspace{-3mm}
\vspace{-10mm}
\subfloat{\includegraphics[width=0.85\linewidth]{latex/figures/Visulization/hist.png}}\end{center}
\vspace{3mm}
\caption{Histogram of standard deviation along each dimension of feature of extracted by pretrained model and our IMRNet model. We show a case of the \textit{Duck} class in Real3D-AD dataset.\textcolor{red}{consider change the front-back relation between IMR and RAW}}
\label{fig:duck}
% 

% 
% We note that the synthesized blurry hand image contains multiple annotations from 3D GTs of \emph{1st}, \emph{3rd}, and \emph{5th} sharp frames.

\vspace{-5mm}

\end{figure}

==> latex/supple/figures/effect.tex <==
% \vspace{-4mm}

% \end{figure}
\begin{figure*}
    \subfloat[Iteration number influence.]{
        \begin{minipage}[t]{0.46\linewidth}
            \centering
            \includegraphics[width=0.9\linewidth]{latex/supple/figures/iteration.png}
            \label{fig:iter}
        \end{minipage}
    }
    \hfill
    \subfloat[Patch size influence.]{
        \begin{minipage}[t]{0.46\linewidth}
            \centering
            \includegraphics[width=0.9\linewidth]{latex/supple/figures/patch.png}
            \label{fig:mask1}
        \end{minipage}
    }
    \vspace{-5pt}
     \caption{Ablation study of iteration number and patch size.}
      \vspace{-5pt}
     \label{fig:patch}
\label{fig:effect}
\end{figure*}

==> latex/supple/figures/vis.tex <==
\begin{figure*}[htp]
\begin{center}
\vspace{-5mm}
\hspace{-5mm}
\subfloat{\includegraphics[width=\linewidth]{latex/supple/figures/3DAD.png}}\end{center}
\vspace{-2mm}
\caption{\textbf{Qualitative results visualization of anomaly localization performance on Real3D-AD.}}
\vspace{-2mm}
\label{fig:vis}
\end{figure*}

==> latex/supple/sections/0_introduction.tex <==
\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{equation}{0}

\renewcommand{\thetable}{S\arabic{table}}
\renewcommand{\thesection}{S\arabic{section}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\theequation}{S\arabic{equation}}

In this supplementary material, we provide 
more details that could not be included in the main manuscript due to the lack of space.
The contents are summarized below:

\begin{compactitem}[$\bullet$]
    \item \ref{sec:samples}. More Anomaly-ShapeNet anomaly samples.
    \item \ref{sec:visualization}.Visualization samples of Real3D-AD for anomaly detection and localization.
    \item \ref{sec:experiments}. Complete experiment results of IMRNet on anomaly detection and segmentation.
    \item \ref{sec:effect}. Ablation Study of iteration number and patch size. 
    \item \ref{sec:discussion}. Limitations and future works.
\end{compactitem}




==> latex/supple/sections/1_samples.tex <==
\section{Anomaly-ShapeNet Samples}
In this section, we present more anomalous examples of our proposed Anomaly-ShapeNet dataset. Figure \ref{s1} and \ref{s2} display the meshes and point clouds legends of six different anomaly types.
\label{sec:samples}
% \input{latex/supple/figures/samples}

==> latex/supple/sections/2_experiments.tex <==
\section{Complete experiment results of IMRNet on anomaly detection and segmentation}
\label{sec:experiments}
To provide a comprehensive benchmark for our Anomaly-ShapeNet dataset, we tested different metrics on the Anomaly-ShapeNet dataset using mainstream 3D algorithms. The experimental results are presented in Table \ref{p-auc} and Table \ref{i-ap}
% \input{latex/supple/tables/P-AUC}
% \input{latex/supple/tables/I-AP}

==> latex/supple/sections/3_visualization.tex <==
\section{Visualization samples of Real3D-AD for anomaly detection and localization.}
\label{sec:visualization}
Within the main text, we showcase a subset of the visualization results for anomaly detection and localization performed by the IMRNet algorithm on Anomaly-ShapeNet. Due to space constraints, the visualizations of IMRNet's detection results on Real-3D are presented in Figure \ref{fig:vis}. In this figure, the detection and localization performance of our IMRNet algorithm is evidently superior to that of the CPMF and RegAD algorithms.
% \input{latex/supple/figures/vis}

==> latex/supple/sections/4_effect.tex <==
\section{Ablation study of iteration number and patch size.}
In the main text, we present the experimental results demonstrating the correlation between the effectiveness of IMRNet's anomaly detection and the masking rate. As a supplement, we provide the relationship curves between anomaly detection performance, mask size, and iteration number in Figure \ref{fig:effect} to aid in understanding the relation of experimental parameters and the detection effect. Figure \ref{fig:effect} demonstrate the best iteration time and patch size are 3 and 64. Theoretically, larger iteration time and patch size may induce normal point drift and increase the positive false rate, while smaller ones may be not enough to cover all anomaly regions. 
\label{sec:effect}
% \input{latex/supple/figures/effect}




==> latex/supple/sections/5_discussion.tex <==
\section{Limitations and future works.}
\label{sec:discussion}

Our proposed Anomaly-ShapeNet dataset, while encompassing a broad distribution of samples, still lacks sufficient scale. Future work will need to focus on expanding the number of samples within the dataset. Moreover, Pure point cloud coordinate-based 3D anomaly detection does not fully conform to real-world 3D anomaly detection scenarios. Subsequent efforts should involve the integration of RGB values into our anomaly detection model.
\input{latex/supple/figures/samples}
\input{latex/supple/figures/vis}
\input{latex/supple/figures/effect}
\input{latex/supple/tables/P-AUC}
\input{latex/supple/tables/I-AP}

==> latex/supple/sections/6_license.tex <==
\subsection*{License of the used assets}
% 

\begin{compactitem}[$\bullet$]
    \item InterHand2.6M dataset~\cite{moon2020interhand2} is CC-BY-NC 4.0 licensed.
    \item YT-3D dataset~\cite{kulon2020weakly} is Ariel AI licensed.
    \item \href{https://github.com/microsoft/MeshTransformer}{METRO~\cite{lin2021end} codes} are released for academic research only and it is free to researchers from educational or research institutes for non-commercial purposes. % code example
    \item \href{https://github.com/mks0601/Hand4Whole_RELEASE}{Pose2Pose~\cite{moon2022accurate} codes} are released for academic research only and it is free to researchers from educational or research institutes for non-commercial purposes. % code example
    \item \href{https://github.com/mks0601/I2L-MeshNet_RELEASE}{I2L-MeshNet~\cite{moon2020i2l} codes} are released for academic research only and it is free to researchers from educational or research institutes for non-commercial purposes. % code example
    
    
\end{compactitem}

\input{latex/supple/figures/YT3D_comparison_first}
\input{latex/supple/figures/BlurHand_comparison.tex}

% \input{latex/supple/figures/YT3D_comparison_last}


==> latex/supple/sections/7_comparison_under_same_cost.tex <==
\section{Number of unfolding under the same cost}
% \label
In Table~\ref{reb_tab:efficiency}, we report the performance of BlurHandNet with different numbers of unfolding steps.
Since the 
For a fair comparison, we keep the number of parameters the same by adjusting the channel size.
The results demonstrate that the performance improvement is not due to a larger network capacity.
% 
\begin{table}[!t]
    \vspace{-3mm}
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        \;~\# of unfolding & 1 & 3~(Ours) & 5\\
        \midrule
        % \,~GMACs~(\jaeha{unit}) & 13.59 & 30.02 & 46.44\\
        % \,~$\#$ of params~(M) &  & 85.36 & 85.39 \\
        \,~MPJPE (middle) & 17.48 & \textbf{16.80} & 16.91\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
    \caption{\textbf{Effects of the number of unfolded hands on the BH.}}
    \label{reb_tab:efficiency}
    \vspace{-4mm}
\end{table}

==> latex/supple/tables/I-AP.tex <==
\begin{table*}
  \vspace{-10pt}
  \centering
  \scriptsize
  \renewcommand\arraystretch{0.55}
  \begin{tabular}{@{}cl|m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.65cm}<{\centering}m{0.65cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering} m{0.6cm}<{\centering}}
    \toprule
    & Method & cap0 & cap3 &helmet3  & cup0 & bowl4 & vase3 & headset1 & eraser0 & vase8 & cap4 &vase2 & vase4 & helmet0 & bucket1\\
    \midrule 
     &BTF(Raw) & 0.659 & 0.612 & 0.526 & 0.601 & 0.601 & 0.717 & 0.515 & 0.425 & 0.416 & 0.515 & 0.413&0.428 &0.559&0.620 \\
     &BTF(FPFH) & 0.618 & 0.579 & 0.564 & 0.585 & 0.632 & 0.652 & 0.523 & 0.719 & 0.624 & 0.545 & 0.569 &0.587 &0.568&0.648 \\
     &M3DM & 0.564 & 0.652 & 0.458 & 0.570 & 0.571 & 0.551 & 0.623 & 0.625 & 0.463 & 0.477 & 0.615&0.526 &0.528&0.507 \\
     &Patchcore(FPFH) & 0.585 & 0.457 & 0.494& 0.604 & 0.575 & 0.481 & 0.601 & 0.584 & 0.515 & 0.655 & 0.801&0.777 &0.525&0.565 \\
     &Patchcore(PointMAE) & 0.561  & 0.583 & 0.611 & 0.642 & 0.601 & 0.455 & 0.423 & 0.801 & 0.655 &0.721 & 0.711&0.586 &0.633&0.642 \\
     &CPMF & 0.601 & 0.541 & 0.645 & 0.647 & 0.683 & 0.588 & 0.619 & 0.544 & 0.673 & 0.645 & 0.632&0.655 &0.333&0.501\\
     &RegAD & 0.693 & 0.711 & 0.468 &0.531& 0.624 & 0.651 & 0.617 & 0.424 & 0.629 & 0.623 & 0.641 & 0.505&0.600 &0.714\\
     &\textbf{Ours} &  0.711 & 0.702 &  0.575 &  0.455 & 0.630 & 0.708  & 0.656 & 0.599 &0.639 & 0.658 &0.655 &0.528 & 0.697&0.732\\
     \midrule
    \midrule
    & Method & bottle3 & vase0 & bottle0 & tap1 & bowl0 & bucket0 & vase5 & vase1 & vase9 & ashtray0 & bottle1 & tap0 & phone & cup1\\
    \midrule 
     &BTF(Raw) & 0.543 & 0.562 & 0.466 & 0.594 & 0.588 & 0.652 & 0.615 & 0.441 & 0.482 & 0.578 & 0.573&0.535 &0.613&0.701 \\
     &BTF(FPFH) & 0.602 & 0.641 & 0.644 & 0.575 & 0.576 & 0.483 & 0.472 & 0.655 & 0.638 & 0.651 & 0.625 &0.610 &0.662&0.651 \\
     &M3DM & 0.451 & 0.788 & 0.763 & 0.638 & 0.525 & 0.609 & 0.633 & 0.652 & 0.651 & 0.632 & 0.674&0.722 &0.464&0.752 \\
     &Patchcore(FPFH) & 0.579 & 0.645 & 0.615&0.684 & 0.548 & 0.604 & 0.515 & 0.623 & 0.660 & 0.445 & 0.677&0.712 &0.332&0.586 \\
     &Patchcore(PointMAE) & 0.651  & 0.548 & 0.545& 0.542 & 0.562 & 0.541 & 0.585 & 0.572 & 0.634 &0.679 & 0.645&0.712 &0.652&0.710 \\
     &CPMF & 0.505 & 0.632 & 0.588 & 0.697 & 0.775 & 0.662 & 0.518 & 0.645 & 0.618 & 0.453 & 0.592&0.639 &0.655&0.609\\
     &RegAD & 0.474 & 0.615 & 0.632 & 0.599 & 0.494 & 0.632 & 0.588 & 0.468 & 0.574 & 0.588 & 0.695&0.676 &0.614&0.638\\
     &\textbf{Ours} & 0.648 & 0.573 &  0.558 & 0.796 &  0.481 & 0.578 & 0.654 & 0.725&0.462&0.612&0.702 & 0.401&0.552 &0.627 \\
    \midrule
    \midrule
    & Method & vase7 & helmet2  & cap5 & shelf0 & bowl5 & bowl3 & helmet1 & bowl1 & headset0 & bag0& bowl2 & jar& \multicolumn{2}{|c}{\textbf{Mean}} \\
    \midrule 
     &BTF(Raw) & 0.547 & 0.615  & 0.653 & 0.624 & 0.615 & 0.654 & 0.388 & 0.464 & 0.379 & 0.458&0.576 &0.428&\multicolumn{2}{|c}{0.549} \\
     &BTF(FPFH) & 0.592 & 0.588  & 0.593 & 0.611 & 0.699 & 0.499 & 0.721 & 0.648 & 0.531 & 0.551 &0.515 &0.479&\multicolumn{2}{|c}{0.598} \\
     &M3DM & 0.648 & 0.636  & 0.642 & 0.665 & 0.601 & 0.635 & 0.627 & 0.515 & 0.632 & 0.642&0.630 &0.555&\multicolumn{2}{|c}{0.603} \\
     &Patchcore(FPFH) & 0.621 & 0.475 & 0.725 & 0.504 & 0.541 & 0.620 & 0.630 & 0.545 & 0.701 & 0.608&0.611 &0.499&\multicolumn{2}{|c}{0.588} \\
     &Patchcore(PointMAE) & 0.652  & 0.496  & 0.542 & 0.543 & 0.585 & 0.556 & 0.571 & 0.611 &0.515 & 0.601&0.456 &0.463&\multicolumn{2}{|c}{0.595} \\
     &CPMF & 0.432 & 0.477  & 0.697 & 0.681 & 0.685 & 0.418 & 0.501 & 0.621 & 0.602 & 0.655&0.601 &0.618&\multicolumn{2}{|c}{0.597}\\
     &RegAD & 0.455& 0.618  & 0.77 &0.675 & 0.555 & 0.441 & 0.381 & 0.515 & 0.538 & 0.608&0.495 &0.601&\multicolumn{2}{|c}{0.584}\\
     &\textbf{Ours} & 0.601 & 0.602 & 0.502 &  0.625 & 0.652 & 0.614 & 0.615& 0.504 & 0.701 &0.665 &0.681 &0.760 & \multicolumn{2}{|c}{0.621}\\
    \bottomrule
  \end{tabular}
  \vspace{-5pt}
  \caption{\textbf{I-AP score for anomaly detection of 40 categories of our Anomaly-ShapeNet dataset}}
  \vspace{-10pt}
  \label{i-ap}
\end{table*}


==> latex/supple/tables/P-AUC.tex <==
\begin{table*}
  \vspace{-10pt}
  \centering
  \scriptsize
  \renewcommand\arraystretch{0.55}
  \begin{tabular}{@{}cl|m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.65cm}<{\centering}m{0.65cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering} m{0.6cm}<{\centering}}
    \toprule
    & Method & cap0 & cap3 &helmet3  & cup0 & bowl4 & vase3 & headset1 & eraser0 & vase8 & cap4 &vase2 & vase4 & helmet0 & bucket1\\
    \midrule 
     &BTF(Raw) & 0.524 & 0.687 & 0.700 & 0.632 & 0.563 & 0.602 & 0.475 & 0.637 & 0.550 & 0.469 & 0.403&0.613 &0.504&0.686 \\
     &BTF(FPFH) & 0.730 & 0.658 & 0.724 & 0.790 & 0.679 & 0.699 & 0.591 & 0.719 & 0.662 & 0.524 & 0.646 &0.710 &0.575&0.633 \\
     &M3DM & 0.531 & 0.605 & 0.655 & 0.715 & 0.624 & 0.658 & 0.585 & 0.710 & 0.551 & 0.718 & 0.737&0.655 &0.599&0.699 \\
     &Patchcore(FPFH) & 0.472 & 0.653 & 0.737& 0.655 & 0.720 & 0.430 & 0.464 & 0.810 & 0.575 & 0.595 & 0.721&0.505 &0.548&0.571 \\
     &Patchcore(PointMAE) & 0.544  & 0.488 & 0.615 & 0.510 & 0.501 & 0.465 & 0.423 & 0.378 & 0.364 &0.725 & 0.742&0.523 &0.580&0.574 \\
     &CPMF & 0.601 & 0.551 & 0.520 & 0.497 & 0.683 & 0.582 & 0.458 & 0.689 & 0.529 & 0.553 & 0.582&0.514 &0.555&0.601\\
     &RegAD & 0.632 & 0.718 & 0.620 &0.685& 0.800 & 0.511 & 0.626 & 0.755 & 0.811 & 0.815 & 0.405 & 0.755&0.600 &0.752\\
     &\textbf{Ours} &  0.715 & 0.706 &  0.663 &  0.643 & 0.576 & 0.401  & 0.476 & 0.548 &0.635 & 0.753 &0.614 &0.524 & 0.598&0.774\\
     \midrule
    \midrule
    & Method & bottle3 & vase0 & bottle0 & tap1 & bowl0 & bucket0 & vase5 & vase1 & vase9 & ashtray0 & bottle1 & tap0 & phone & cup1\\
    \midrule 
     &BTF(Raw) & 0.720 & 0.618 & 0.551 & 0.564 & 0.524 & 0.617 & 0.585 & 0.549 & 0.564 & 0.512 & 0.491&0.527 &0.583&0.561 \\
     &BTF(FPFH) & 0.622 & 0.642 & 0.641 & 0.596 & 0.710 & 0.401 & 0.429 & 0.619 & 0.568 & 0.624 & 0.549 &0.568 &0.675&0.619 \\
     &M3DM & 0.532 & 0.608 & 0.663 & 0.712 & 0.658 & 0.698 & 0.642 & 0.602 & 0.663 & 0.577 & 0.637&0.654 &0.358&0.556 \\
     &Patchcore(FPFH) & 0.512 & 0.655 & 0.654& 0.768 & 0.524 & 0.459 & 0.447 & 0.453 & 0.663 & 0.597 & 0.687&0.733 &0.488&0.596 \\
     &Patchcore(PointMAE) & 0.653  & 0.677 & 0.553 & 0.541 & 0.527 & 0.586 & 0.572 & 0.551 & 0.423 &0.495 & 0.606&0.858 &0.886&0.856 \\
     &CPMF & 0.435 & 0.458 & 0.521 & 0.657 & 0.745 & 0.486 & 0.651 & 0.486 & 0.545 & 0.615 & 0.571&0.458 &0.545&0.509\\
     &RegAD & 0.525 & 0.548 & 0.886 & 0.741 & 0.775 & 0.619 & 0.624 & 0.602 & 0.694 & 0.698 & 0.696&0.589 &0.599&0.698\\
     &\textbf{Ours} & 0.641 & 0.535 &  0.556 & 0.699 &  0.781 & 0.585 & 0.682 & 0.685&0.691&0.671&0.702 & 0.681&0.742&0.688 \\
    \midrule
    \midrule
    & Method & vase7 & helmet2  & cap5 & shelf0 & bowl5 & bowl3 & helmet1 & bowl1 & headset0 & bag0& bowl2 & jar& \multicolumn{2}{|c}{\textbf{Mean}} \\
    \midrule 
     &BTF(Raw) & 0.578 & 0.605  & 0.373 & 0.464 & 0.517 & 0.685 & 0.449 & 0.464 & 0.578 & 0.430&0.426 &0.423&\multicolumn{2}{|c}{0.550} \\
     &BTF(FPFH) & 0.540 & 0.643  & 0.586 & 0.619 & 0.699 & 0.590 & 0.749 & 0.768 & 0.620 & 0.746 &0.518 &0.427&\multicolumn{2}{|c}{0.628} \\
     &M3DM & 0.517 & 0.623  & 0.655 & 0.554 & 0.489 & 0.657 & 0.427 & 0.663 & 0.581 & 0.637&0.694 &0.541&\multicolumn{2}{|c}{0.616} \\
     &Patchcore(FPFH) & 0.693 & 0.455 &  0.795 & 0.613 & 0.358 & 0.327 & 0.489 & 0.531 & 0.583 & 0.574&0.625 &0.478&\multicolumn{2}{|c}{0.580} \\
     &Patchcore(PointMAE) & 0.651  & 0.651  & 0.545 & 0.543 & 0.562 & 0.581 & 0.562 & 0.524 &0.575 & 0.674&0.515 &0.487&\multicolumn{2}{|c}{0.577} \\
     &CPMF & 0.504 & 0.515  & 0.551 & 0.783 & 0.684 & 0.641 & 0.542 & 0.488 & 0.699 & 0.655&0.635&0.611&\multicolumn{2}{|c}{0.573}\\
     &RegAD & 0.881& 0.825  & 0.467 &0.688 & 0.691 & 0.654 & 0.624 & 0.615 & 0.580 & 0.715&0.593 &0.599&\multicolumn{2}{|c}{0.668}\\
     &\textbf{Ours} & 0.593 & 0.644  & 0.742 &  0.605 &0.715 & 0.599 & 0.604& 0.705 &  0.705 &0.668 &0.684 &0.765 & \multicolumn{2}{|c}{0.650}\\
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \caption{\textbf{P-AUROC score for anomaly detection of 40 categories of our Anomaly-ShapeNet dataset}}
  \vspace{-10pt}
  \label{p-auc}
\end{table*}

==> latex/tables/5.3/Ablation_of_iteration.tex <==
\begin{table}
  \centering
  \scriptsize
  \begin{tabularx}{0.8\linewidth}{@{}l|ccc|}
    \toprule
    Iter num  & I-AUROC & I-AP & P-AUROC\\
    \midrule
    1 & 0.796 & 0.927 & 0.981 \\
    2 & 0.821 & 0.939 & 0.985 \\
    3 & 0.903 & 0.953 & 0.988 \\
    4  & 0.945 & 0.964 &  0.992  \\
    \bottomrule
  \end{tabularx}
  \vspace{-5pt}
  \caption{\textbf{Ablation study on the number of iteration.}}
  \vspace{-10pt}
  \label{tab:iteration}
\end{table}

==> latex/tables/5.3/iteration.tex <==
% \begin{table}[!t]
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{C{1.6cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% \# of  &  \multicolumn{5}{c}{MPJPE} \\
% \cline{2-6}
% unfolding & initial & initial$^*$ & middle & final$^*$ & final \\
% \hline
% 1 & - & - & 17.41 & - & - \\
% \textbf{3 (Ours)} & 18.08 & - & 16.80 & - & 18.21 \\
% 5 & 18.06 & 17.18 & 16.78 & 17.36 & 18.18 \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}}
% \vspace{-3mm}
% \caption{
%     \textbf{Effects of number of unfolded hands on BlurHand dataset.}
%     The notation $^*$ denotes hands between the middle and both ends of motion.
% }
% \vspace{-3mm}
% \label{table:unfoldingnumber}
% \end{table}


\begin{table}[!t]
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{L{2.0cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}|C{1.1cm}}
\specialrule{.1em}{.05em}{.05em}
\hline
% \,~\multirow{2}{*}{\# of unfolding} &  \multicolumn{5}{c}{MPJPE} \\
% \cline{2-6}
%  & initial & initial$^*$ & middle & final$^*$ & final \\
\,~\multirow{2}{*}{\# iteration } &  \multicolumn{5}{c}{Metrics} \\
\cline{2-6}
& I-AUC & P-AUC & I-AP & P-AP & Time \\
\hline
\;~1 & - & - & 17.41 & - & - \\
\;~2 & 18.08 & - & 16.80 & - & 18.21 \\
\;~\textbf{3} & 18.06 & 17.18 & 16.78 & 17.36 & 18.18 \\
\;~4 & 18.06 & 17.18 & 16.78 & 17.36 & 18.18 \\
\hline
\specialrule{.1em}{.05em}{.05em}
\end{tabular}}
\vspace{-3mm}
\caption{
    % \textbf{Effects of number of unfolded hands on BlurHand dataset.}
    % \textbf{Effects of the number of unfolded hands.}
    \textbf{Ablation study on the number of iteration.}
    % The notation $^*$ denotes hands between the middle and both ends of motion.
    The bold number represents the iteration number corresponding to the highest I-AUC. I-AUC,P-AUC are image and pixel level average AUROC. I-AP and P-AP are image and pixel level average precision. Time is the testing time of corresponding iteration number. 
}
\vspace{-3mm}
\label{table:iteration}
\end{table}
